Semantic Semi-Incremental Data-Association-Free Object SLAM

Data association between landmark measurements and landmark variables has long been a central challenge in SLAM, as estimation accuracy depends critically on associating measurements with the correct landmark variables. Recent advances in deep learning have created new opportunities for the problem; data association can now leverage not only positional measurements but also semantic information about object landmarks, such as class labels from neural object detectors and feature vectors from visual foundation models. In this paper, we present a generalized data-association-free SLAM framework that jointly estimates data associations, robot poses, landmark positions, and landmark semantics from odometry, and positional and semantic measurements of landmarks. The proposed framework (i) creates a synergy between data association and landmark semantics estimation; (ii) adopts a semi-incremental estimation scheme for improved accuracy and computational efficiency; and (iii) provides a principled justification, guidelines, and heuristics for landmark-number estimation, improving the interpretability and practical usability of the framework. The proposed framework and algorithms are evaluated on synthetic and real-world datasets with two types of semantic information, class labels and real-valued feature vectors, and demonstrate superior performance compared to strong baselines.

==> includes/scripts/proof_draft_dloghlesszero.tex <==
\paragraph{Proof of the Gaussian tail inequality.}

We prove the inequality
\begin{equation}
\phi(t)\left(\frac{1}{\bar{\Phi}(t)}-\frac{1}{\Phi(t)}\right)<2t,
\qquad t>0,
\end{equation}
which is used to show that
\[
h(t)=\frac{\phi(t)^2}{\Phi(t)\bar{\Phi}(t)}
\]
is decreasing for \(t>0\).

First, define the inverse Mills ratio
\begin{equation}
\lambda(x)=\frac{\phi(x)}{\bar{\Phi}(x)}.
\end{equation}

Using the symmetry of the standard Gaussian,
\[
\phi(-x)=\phi(x),
\qquad
\bar{\Phi}(-x)=\Phi(x),
\]
we obtain
\[
\lambda(-x)=\frac{\phi(x)}{\Phi(x)}.
\]
Therefore,
\begin{equation}
\phi(t)\left(\frac{1}{\bar{\Phi}(t)}-\frac{1}{\Phi(t)}\right)
=
\lambda(t)-\lambda(-t).
\end{equation}

Next, differentiate the inverse Mills ratio:
\[
\lambda'(x)
=
\frac{\phi'(x)\bar{\Phi}(x)-\phi(x)\bar{\Phi}'(x)}
{\bar{\Phi}(x)^2}.
\]
Since
\[
\phi'(x)=-x\phi(x),
\qquad
\bar{\Phi}'(x)=-\phi(x),
\]
it follows that
\begin{align}
\lambda'(x)
&=
\frac{-x\phi(x)\bar{\Phi}(x)+\phi(x)^2}
{\bar{\Phi}(x)^2} \\
&=
\frac{\phi(x)}{\bar{\Phi}(x)}
\left(
\frac{\phi(x)}{\bar{\Phi}(x)}-x
\right) \\
&=
\lambda(x)\bigl(\lambda(x)-x\bigr).
\end{align}

To bound this derivative, let \(Z\sim\mathcal N(0,1)\). The conditional mean of the truncated Gaussian is
\[
E[Z\mid Z>x]
=
\frac{\int_x^\infty z\phi(z)\,dz}
{\bar{\Phi}(x)}
=
\frac{\phi(x)}{\bar{\Phi}(x)}
=
\lambda(x),
\]
where we used
\[
\int_x^\infty z\phi(z)\,dz=\phi(x).
\]

Similarly,
\[
E[Z^2\mid Z>x]
=
\frac{\int_x^\infty z^2\phi(z)\,dz}
{\bar{\Phi}(x)}.
\]
Integration by parts gives
\[
\int_x^\infty z^2\phi(z)\,dz
=
x\phi(x)+\bar{\Phi}(x),
\]
so that
\[
E[Z^2\mid Z>x]
=
1+x\lambda(x).
\]

Hence,
\begin{align}
\operatorname{Var}(Z\mid Z>x)
&=
E[Z^2\mid Z>x]
-
E[Z\mid Z>x]^2 \\
&=
1+x\lambda(x)-\lambda(x)^2.
\end{align}

Since a variance is nonnegative,
\[
1+x\lambda(x)-\lambda(x)^2\ge0,
\]
which implies
\[
\lambda(x)^2-x\lambda(x)\le1.
\]
Using the expression for \(\lambda'(x)\),
\[
\boxed{
\lambda'(x)\le1.
}
\]
In fact, the inequality is strict because
\(\operatorname{Var}(Z\mid Z>x)>0\), so
\[
\lambda'(x)<1.
\]

Finally, integrate over the interval \([-t,t]\):
\begin{align}
\lambda(t)-\lambda(-t)
&=
\int_{-t}^{t}\lambda'(x)\,dx \\
&<
\int_{-t}^{t}1\,dx \\
&=
2t.
\end{align}

Substituting back yields
\[
\boxed{
\phi(t)
\left(
\frac{1}{\bar{\Phi}(t)}
-
\frac{1}{\Phi(t)}
\right)
<
2t,
\qquad t>0.
}
\]

Consequently,
\[
\frac{d}{dt}\log h(t)
=
-2t
+
\phi(t)
\left(
\frac{1}{\bar{\Phi}(t)}
-
\frac{1}{\Phi(t)}
\right)
<
0,
\]
showing that \(h(t)\) is strictly decreasing for \(t>0\). Since \(h(t)\) is an even function, it attains its maximum at \(t=0\).

==> includes/scripts/proof_draft_hfsplit_optim.tex <==
\subsection{Optimality of the Half-Space Split}
\label{app: half_space_optimality}

We now show that the centered half-space split considered above is
population-optimal under the idealized whitened Gaussian splitting model.
Recall from Lemma~1 that, for any binary split of \(n\) measurements into
two nonempty groups \(G_1\) and \(G_2\),
\[
r_0-r_{\rm split}
=
\frac{n_1n_2}{n}
\|\bar u_1-\bar u_2\|^2 .
\]
This expression contains two coupled effects: the balance of the split,
through \(n_1n_2/n\), and the separation between the group means, through
\(\|\bar u_1-\bar u_2\|^2\). Therefore, optimality cannot be argued from
the balance term alone.

We analyze the population analogue. Let
\[
U\sim\mathcal N(0,I_d)
\]
be a centered and whitened residual from one landmark cluster. Consider
any measurable binary split of the space into \(A\) and \(A^c\), and define
\[
p=\mathbb P(U\in A),\qquad
m_A=\mathbb E[U\mid U\in A],\qquad
m_{A^c}=\mathbb E[U\mid U\in A^c].
\]
The population residual reduction corresponding to Lemma~1 is
\[
\mathcal R(A)
=
p(1-p)\|m_A-m_{A^c}\|^2 .
\]
Because \(U\) is centered, the law of total expectation gives
\[
0=\mathbb E[U]
=
p m_A+(1-p)m_{A^c}.
\]
Hence,
\[
m_{A^c}
=
-\frac{p}{1-p}m_A.
\]
Therefore,
\[
m_A-m_{A^c}
=
\frac{1}{1-p}m_A,
\]
and
\[
\mathcal R(A)
=
\frac{p}{1-p}\|m_A\|^2 .
\]

At this point, \(p\) and \(m_A\) are both determined by the choice of
\(A\). We decompose the joint optimization exactly by grouping all
regions according to their probability mass:
\[
\max_A \mathcal R(A)
=
\max_{0<p<1}
\max_{A:\mathbb P(U\in A)=p}
\mathcal R(A).
\]
This is not a coordinate-wise approximation; every feasible region \(A\)
has a unique mass \(p=\mathbb P(U\in A)\). Fixing \(p\) fixes only the
amount of probability mass selected, not the conditional mean \(m_A\).

For fixed \(p\), the factor \(p/(1-p)\) is constant. Therefore, the inner
problem is equivalent to
\[
\max_{A:\mathbb P(U\in A)=p}\|m_A\|.
\]
Let \(A\) be any candidate region with \(m_A\neq 0\), and define
\[
a=\frac{m_A}{\|m_A\|}.
\]
Then
\[
\|m_A\|
=
a^\top m_A.
\]
Using
\[
m_A
=
\mathbb E[U\mid U\in A]
=
\frac{\mathbb E[U\mathbf 1_A]}{\mathbb P(U\in A)}
=
\frac{1}{p}\mathbb E[U\mathbf 1_A],
\]
we obtain
\[
\|m_A\|
=
\frac{1}{p}\mathbb E[a^\top U\mathbf 1_A].
\]
Let \(S=a^\top U\). Since \(U\sim\mathcal N(0,I_d)\) and
\(\|a\|=1\), we have
\[
S\sim\mathcal N(0,1).
\]
For fixed \(p\), maximizing \(\|m_A\|\) is therefore equivalent to
maximizing
\[
\mathbb E[S\mathbf 1_A]
\]
over all regions \(A\) satisfying \(\mathbb P(U\in A)=p\). This is
achieved by selecting the points with the largest values of \(S\). If a
region contains a point with smaller \(S\) while excluding a point with
larger \(S\), swapping them increases the expectation without changing
the probability mass. Therefore, the optimal fixed-\(p\) region is an
upper-level set of \(S\), namely a half-space
\[
A_t=\{U:a^\top U\ge t\},
\]
where \(t\) satisfies
\[
p=\mathbb P(a^\top U\ge t)=\bar\Phi(t).
\]

For this half-space,
\[
\mathbb E[S\mathbf 1_{S\ge t}]
=
\int_t^\infty s\phi(s)\,ds.
\]
Since \(\phi'(s)=-s\phi(s)\), we have
\[
\int_t^\infty s\phi(s)\,ds
=
\phi(t).
\]
Thus,
\[
\|m_{A_t}\|
=
\frac{\phi(t)}{\bar\Phi(t)}.
\]
Substituting this into
\[
\mathcal R(A)=\frac{p}{1-p}\|m_A\|^2
\]
with \(p=\bar\Phi(t)\) and \(1-p=\Phi(t)\), we obtain
\[
\mathcal R(A_t)
=
\frac{\phi(t)^2}{\Phi(t)\bar\Phi(t)}.
\]
Thus, the original split optimization reduces to the one-dimensional
problem
\[
\max_t h(t),
\qquad
h(t)=\frac{\phi(t)^2}{\Phi(t)\bar\Phi(t)}.
\]

The function \(h(t)\) is symmetric around \(t=0\). Differentiating
\(\log h(t)\) gives
\[
\frac{d}{dt}\log h(t)
=
-2t
+
\phi(t)
\left(
\frac{1}{\bar\Phi(t)}
-
\frac{1}{\Phi(t)}
\right).
\]
For \(t>0\), this derivative is negative by the standard Gaussian
Mills-ratio inequality
\[
\phi(t)
\left(
\frac{1}{\bar\Phi(t)}
-
\frac{1}{\Phi(t)}
\right)
<
2t.
\]
By symmetry, the derivative is positive for \(t<0\). Therefore,
\(h(t)\) is maximized at \(t=0\), which corresponds to
\[
p=\bar\Phi(0)=\frac{1}{2}.
\]
The optimal split is therefore the centered half-space
\[
A^\star=\{U:a^\top U\ge 0\}.
\]

At \(t=0\),
\[
\phi(0)=\frac{1}{\sqrt{2\pi}},
\qquad
\Phi(0)=\bar\Phi(0)=\frac{1}{2}.
\]
Hence,
\[
\max_A \mathcal R(A)
=
\frac{\phi(0)^2}{\Phi(0)\bar\Phi(0)}
=
\frac{1/(2\pi)}{1/4}
=
\frac{2}{\pi}.
\]
Consequently, for \(n\) i.i.d. whitened Gaussian measurements,
\[
\max_{G_1,G_2}
(r_0-r_{\rm split})
\approx
\frac{2n}{\pi},
\]
or equivalently,
\[
\frac{1}{n}
\max_{G_1,G_2}
(r_0-r_{\rm split})
\rightarrow
\frac{2}{\pi}
\qquad
\text{as}
\qquad
n\rightarrow\infty.
\]
This proves that the centered half-space split is population-optimal
under the idealized whitened Gaussian model.

==> includes/scripts/proof_draft_rand_hf_splits.tex <==
\section*{Splitting A Large Number of Gaussian Samples}
\label{app: split_reduction}
Following up on the previous section "Low Inter-Landmark Spacing Scenario", we model the addition of a landmark as splitting Gaussian samples to approximate the objective value change from $\fslamstar{K^\star}$ to the pre-optimization (non-optimal) value of $\fslam(K^\star + 1)$. Fig. \ref{fig: splitsamples} shows a schematic for illustration. For clarity, we hereafter use unique notations that are independent from the rest of the paper.
\input{includes/scripts/fig_splitsamples}

\subsection{Problem Setup}

Consider one true landmark observed \(n\) times. Let $u_1,\ldots,u_n\in\R^d$ denote the whitened measurement samples for this landmark after subtracting the unknown true landmark position. We assume
\[
u_1,\ldots,u_n \overset{\text{i.i.d.}}{\sim} \mathcal N(0,I_d).
\]

Importantly, the vectors \(u_i\) are not yet the residuals used by the optimized
SLAM/k-means objective. In the SLAM objective, the landmark position is an
estimated variable. Therefore, for a fixed set of measurements assigned to one
landmark, the best one-cluster center is the sample mean
\[
\bar u
=
\frac{1}{n}\sum_{i=1}^{n}u_i .
\]
Thus, the optimized one-cluster residual is
\[
r_0
=
\min_{c\in\R^d}\sum_{i=1}^{n}\|u_i-c\|^2
=
\sum_{i=1}^{n}\|u_i-\bar u\|^2 .
\]

If the true landmark center were known and fixed,
then the residual would be
\[
\sum_{i=1}^{n}\|u_i\|^2.
\]
However, in the SLAM/k-means setting, the landmark center is fitted from the
data, so the relevant one-cluster residual is
\[
r_0
=
\sum_{i=1}^{n}\|u_i-\bar u\|^2 .
\]

Since one \(d\)-dimensional mean is estimated, the residual has
\[
d(n-1)
\]
degrees of freedom:
\[
r_0\sim \chi^2_{d(n-1)}.
\]
Therefore,
\[
\E[r_0]=d(n-1).
\]
For large \(n\),
\[
r_0\approx nd.
\]

In the 3D landmark case,
\[
d=3,
\]
so
\[
\E[r_0]=3(n-1),
\qquad
r_0\approx 3n.
\]


\subsection{Reduction Formula for Any Fixed Split}

Suppose the measurements are split into two nonempty groups
\[
G_1,\qquad G_2,
\]
with sizes
\[
n_1=|G_1|,
\qquad
n_2=|G_2|,
\qquad
n_1+n_2=n.
\]
Define the two fitted group centers
\[
\mu_1
=
\frac{1}{n_1}\sum_{i\in G_1}u_i,
\qquad
\mu_2
=
\frac{1}{n_2}\sum_{i\in G_2}u_i.
\]
After splitting the cluster into two clusters, the optimized two-cluster residual is
\[
r_{\rm split}
=
\sum_{i\in G_1}\|u_i-\mu_1\|^2
+
\sum_{i\in G_2}\|u_i-\mu_2\|^2 .
\]


\begin{lemma}[Reduction from one fitted center to two fitted centers]
For any fixed split \(G_1,G_2\),
\[
r_0-r_{\rm split}
=
n_1\|\mu_1-\bar u\|^2
+
n_2\|\mu_2-\bar u\|^2 .
\]
Equivalently,
\[
r_0-r_{\rm split}
=
\frac{n_1n_2}{n}\|\mu_1-\mu_2\|^2 .
\]
\end{lemma}


\begin{proof}
We prove the identity directly by expanding the squared norms.

For any \(i\in G_1\), add and subtract \(\mu_1\):
\[
u_i-\bar u
=
(u_i-\mu_1)+(\mu_1-\bar u).
\]
Therefore,
\[
\|u_i-\bar u\|^2
=
\|(u_i-\mu_1)+(\mu_1-\bar u)\|^2.
\]

We obtain
\[
\|u_i-\bar u\|^2
=
\|u_i-\mu_1\|^2
+
2(u_i-\mu_1)^\top(\mu_1-\bar u)
+
\|\mu_1-\bar u\|^2 .
\]
Now sum this identity over all \(i\in G_1\):
\[
\sum_{i\in G_1}\|u_i-\bar u\|^2
=
\sum_{i\in G_1}\|u_i-\mu_1\|^2
+
2\sum_{i\in G_1}(u_i-\mu_1)^\top(\mu_1-\bar u)
+
\sum_{i\in G_1}\|\mu_1-\bar u\|^2 .
\]

The middle term becomes zero by using the definition of \(\mu_1\):
\[
\mu_1
=
\frac{1}{n_1}\sum_{i\in G_1}u_i .
\]
Hence,
\[
\sum_{i\in G_1}u_i=n_1\mu_1.
\]
Since \(\mu_1\) is constant with respect to \(i\),
\[
\sum_{i\in G_1}\mu_1=n_1\mu_1.
\]
Therefore,
\[
\sum_{i\in G_1}(u_i-\mu_1)
=
\sum_{i\in G_1}u_i-\sum_{i\in G_1}\mu_1
=
n_1\mu_1-n_1\mu_1
=
0.
\]
Thus,
\[
2\sum_{i\in G_1}(u_i-\mu_1)^\top(\mu_1-\bar u)
=
2\left(\sum_{i\in G_1}(u_i-\mu_1)\right)^\top(\mu_1-\bar u)
=
0.
\]

The last term simplifies because \(\mu_1-\bar u\) does not depend on \(i\):
\[
\sum_{i\in G_1}\|\mu_1-\bar u\|^2
=
n_1\|\mu_1-\bar u\|^2.
\]
Therefore,
\[
\sum_{i\in G_1}\|u_i-\bar u\|^2
=
\sum_{i\in G_1}\|u_i-\mu_1\|^2
+
n_1\|\mu_1-\bar u\|^2 .
\]

The same argument for group \(G_2\) gives
\[
\sum_{i\in G_2}\|u_i-\bar u\|^2
=
\sum_{i\in G_2}\|u_i-\mu_2\|^2
+
n_2\|\mu_2-\bar u\|^2 .
\]

Adding the two group identities gives
\[
\sum_{i\in G_1}\|u_i-\bar u\|^2
+
\sum_{i\in G_2}\|u_i-\bar u\|^2
=
\sum_{i\in G_1}\|u_i-\mu_1\|^2
+
\sum_{i\in G_2}\|u_i-\mu_2\|^2
+
n_1\|\mu_1-\bar u\|^2
+
n_2\|\mu_2-\bar u\|^2 .
\]
Since \(G_1\) and \(G_2\) partition all \(n\) samples, the left-hand side is
\[
\sum_{i=1}^{n}\|u_i-\bar u\|^2
=
r_0.
\]
The first two terms on the right-hand side are
\[
\sum_{i\in G_1}\|u_i-\mu_1\|^2
+
\sum_{i\in G_2}\|u_i-\mu_2\|^2
=
r_{\rm split}.
\]
Therefore,
\[
r_0
=
r_{\rm split}
+
n_1\|\mu_1-\bar u\|^2
+
n_2\|\mu_2-\bar u\|^2 .
\]
Rearranging,
\[
r_0-r_{\rm split}
=
n_1\|\mu_1-\bar u\|^2
+
n_2\|\mu_2-\bar u\|^2 .
\]

It remains to prove the equivalent expression in terms of
\(\|\mu_1-\mu_2\|^2\). Since
\[
\bar u
=
\frac{1}{n}\sum_{i=1}^{n}u_i,
\]
and the samples are split into \(G_1\) and \(G_2\), we have
\[
\bar u
=
\frac{1}{n}
\left(
\sum_{i\in G_1}u_i+\sum_{i\in G_2}u_i
\right).
\]
Using
\[
\sum_{i\in G_1}u_i=n_1\mu_1,
\qquad
\sum_{i\in G_2}u_i=n_2\mu_2,
\]
we get
\[
\bar u
=
\frac{n_1\mu_1+n_2\mu_2}{n}.
\]

Now,
\[
\mu_1-\bar u
=
\mu_1-\frac{n_1\mu_1+n_2\mu_2}{n}.
\]
Writing \(\mu_1=n\mu_1/n\), this becomes
\[
\mu_1-\bar u
=
\frac{n\mu_1-n_1\mu_1-n_2\mu_2}{n}.
\]
Since \(n=n_1+n_2\),
\[
n\mu_1-n_1\mu_1
=
n_2\mu_1.
\]
Therefore,
\[
\mu_1-\bar u
=
\frac{n_2\mu_1-n_2\mu_2}{n}
=
\frac{n_2}{n}(\mu_1-\mu_2).
\]
Similarly,
\[
\mu_2-\bar u
=
\mu_2-\frac{n_1\mu_1+n_2\mu_2}{n}
=
\frac{n\mu_2-n_1\mu_1-n_2\mu_2}{n}.
\]
Again using \(n=n_1+n_2\),
\[
n\mu_2-n_2\mu_2
=
n_1\mu_2,
\]
so
\[
\mu_2-\bar u
=
\frac{n_1\mu_2-n_1\mu_1}{n}
=
-\frac{n_1}{n}(\mu_1-\mu_2).
\]

Substitute these two identities into the first expression for the reduction:
\[
r_0-r_{\rm split}
=
n_1
\left\|
\frac{n_2}{n}(\mu_1-\mu_2)
\right\|^2
+
n_2
\left\|
-\frac{n_1}{n}(\mu_1-\mu_2)
\right\|^2 .
\]
Using \(\|a x\|^2=a^2\|x\|^2\), we obtain
\[
r_0-r_{\rm split}
=
n_1
\left(\frac{n_2}{n}\right)^2
\|\mu_1-\mu_2\|^2
+
n_2
\left(\frac{n_1}{n}\right)^2
\|\mu_1-\mu_2\|^2 .
\]
Factor out \(\|\mu_1-\mu_2\|^2\):
\[
r_0-r_{\rm split}
=
\left[
\frac{n_1n_2^2}{n^2}
+
\frac{n_2n_1^2}{n^2}
\right]
\|\mu_1-\mu_2\|^2 .
\]
The coefficient simplifies as
\[
\frac{n_1n_2^2}{n^2}
+
\frac{n_2n_1^2}{n^2}
=
\frac{n_1n_2}{n^2}(n_2+n_1).
\]
Since \(n_1+n_2=n\),
\[
\frac{n_1n_2}{n^2}(n_2+n_1)
=
\frac{n_1n_2}{n^2}n
=
\frac{n_1n_2}{n}.
\]
Therefore,
\[
r_0-r_{\rm split}
=
\frac{n_1n_2}{n}\|\mu_1-\mu_2\|^2 .
\]
This completes the proof.
\end{proof}

Define the residual reduction as
\[
R
:=
r_0-r_{\rm split}.
\]
Then
\[
R
=
n_1\|\mu_1-\bar u\|^2
+
n_2\|\mu_2-\bar u\|^2
=
\frac{n_1n_2}{n}\|\mu_1-\mu_2\|^2 .
\]
Thus, splitting one fitted cluster into two fitted clusters reduces the residual
exactly by the weighted squared separation between the two fitted centers.

\subsection{Case 1: Random Split}

First consider a random split whose group memberships are chosen independently
of the measurement samples. Assume the group sizes \(n_1,n_2\) are fixed.

Because the split is independent of the data, each group contains independent
samples from the same distribution:
\[
u_i\sim \mathcal N(0,I_d).
\]
For group \(G_1\),
\[
\mu_1
=
\frac{1}{n_1}\sum_{i\in G_1}u_i.
\]
A sum of independent Gaussian vectors is Gaussian. Since each \(u_i\) has mean
zero and covariance \(I_d\),
\[
\sum_{i\in G_1}u_i
\sim
\mathcal N(0,n_1 I_d).
\]
Dividing by \(n_1\),
\[
\mu_1
\sim
\mathcal N\left(0,\frac{1}{n_1}I_d\right).
\]
Similarly,
\[
\mu_2
\sim
\mathcal N\left(0,\frac{1}{n_2}I_d\right).
\]
Because the two groups are disjoint and the original samples are independent,
\(\mu_1\) and \(\mu_2\) are independent. Therefore,
\[
\mu_1-\mu_2
\sim
\mathcal N\left(
0,
\left(\frac{1}{n_1}+\frac{1}{n_2}\right)I_d
\right).
\]

For a zero-mean Gaussian vector \(Z\sim\mathcal N(0,\alpha I_d)\),
\[
\E[\|Z\|^2]
=
\sum_{\ell=1}^{d}\E[Z_\ell^2]
=
\sum_{\ell=1}^{d}\alpha
=
d\alpha.
\]
Here,
\[
\alpha
=
\frac{1}{n_1}+\frac{1}{n_2}.
\]
Thus,
\[
\E\left[\|\mu_1-\mu_2\|^2\right]
=
d\left(\frac{1}{n_1}+\frac{1}{n_2}\right).
\]

Using the exact reduction formula,
\[
R_{\rm rand}
=
\frac{n_1n_2}{n}\|\mu_1-\mu_2\|^2 .
\]
Taking expectation,
\[
\E[R_{\rm rand}]
=
\frac{n_1n_2}{n}
\E\left[\|\mu_1-\mu_2\|^2\right].
\]
Substituting the expression above,
\[
\E[R_{\rm rand}]
=
\frac{n_1n_2}{n}
d\left(\frac{1}{n_1}+\frac{1}{n_2}\right).
\]
Now simplify:
\[
\frac{n_1n_2}{n}
\left(\frac{1}{n_1}+\frac{1}{n_2}\right)
=
\frac{n_1n_2}{n}
\left(\frac{n_2+n_1}{n_1n_2}\right)
=
\frac{n_1+n_2}{n}.
\]
Since \(n_1+n_2=n\),
\[
\frac{n_1+n_2}{n}=1.
\]
Therefore,
\[
\boxed{
\E[R_{\rm rand}]=d.
}
\]

Since
\[
\E[r_0]=d(n-1),
\]
the ratio of expectations is
\[
\frac{\E[R_{\rm rand}]}{\E[r_0]}
=
\frac{d}{d(n-1)}
=
\frac{1}{n-1}.
\]
For large \(n\),
\[
\boxed{
\frac{\E[R_{\rm rand}]}{\E[r_0]}
\approx
\frac{1}{n}.
}
\]

For \(d=3\),
\[
\boxed{
\E[R_{\rm rand}]=3,
\qquad
\frac{\E[R_{\rm rand}]}{\E[r_0]}
=
\frac{1}{n-1}
\approx
\frac{1}{n}.
}
\]

\begin{remark}
A random split reduces only \(O(1)\) residual, whereas the one-cluster residual
is \(O(n)\). Therefore, the fractional residual reduction from a random split
vanishes as \(n\to\infty\).
\end{remark}

\subsection{Case 2: Geometric Half-Space Split}

Now consider a geometric split. Choose a unit vector
\[
v\in\R^d,
\qquad
\|v\|=1.
\]
Define the scalar projection
\[
s_i
=
v^\top u_i.
\]
Since
\[
u_i\sim \mathcal N(0,I_d),
\]
we have
\[
s_i\sim \mathcal N(0,1).
\]

Split the samples according to the sign of this projection:
\[
G_+
=
\{i:v^\top u_i>0\},
\qquad
G_-
=
\{i:v^\top u_i<0\}.
\]

Let
\[
s\sim \mathcal N(0,1).
\]
We first compute the conditional mean
\[
\E[s\mid s>0].
\]
By definition,
\[
\E[s\mid s>0]
=
\frac{
\int_0^\infty s\frac{1}{\sqrt{2\pi}}
\exp\left(-\frac{s^2}{2}\right)ds
}{
\mathbb P(s>0)
}.
\]
Since
\[
\mathbb P(s>0)=\frac12,
\]
we get
\[
\E[s\mid s>0]
=
2\int_0^\infty s\frac{1}{\sqrt{2\pi}}
\exp\left(-\frac{s^2}{2}\right)ds.
\]
Let
\[
q=\frac{s^2}{2},
\qquad
dq=s\,ds.
\]
Then
\[
\E[s\mid s>0]
=
\frac{2}{\sqrt{2\pi}}
\int_0^\infty e^{-q}dq.
\]
Since
\[
\int_0^\infty e^{-q}dq=1,
\]
we obtain
\[
\E[s\mid s>0]
=
\sqrt{\frac{2}{\pi}}.
\]
By symmetry,
\[
\E[s\mid s<0]
=
-\sqrt{\frac{2}{\pi}}.
\]

Next, decompose each sample into the component along \(v\) and the component
orthogonal to \(v\):
\[
u=sv+z,
\qquad
z\perp v.
\]
Because the Gaussian distribution is isotropic, the orthogonal component has
zero conditional mean after conditioning on the sign of \(s\):
\[
\E[z\mid s>0]=0,
\qquad
\E[z\mid s<0]=0.
\]
Therefore,
\[
\E[u\mid v^\top u>0]
=
\E[sv+z\mid s>0]
=
\E[s\mid s>0]v+\E[z\mid s>0]
=
\sqrt{\frac{2}{\pi}}v.
\]
Similarly,
\[
\E[u\mid v^\top u<0]
=
-\sqrt{\frac{2}{\pi}}v.
\]

At the population level,
\[
\mu_+
=
\sqrt{\frac{2}{\pi}}v,
\qquad
\mu_-
=
-\sqrt{\frac{2}{\pi}}v,
\]
and the parent mean is
\[
\E[u]=0.
\]
Therefore,
\[
\|\mu_+\|^2
=
\frac{2}{\pi},
\qquad
\|\mu_-\|^2
=
\frac{2}{\pi}.
\]

For large \(n\), approximately half the samples fall into each group:
\[
n_+\approx \frac{n}{2},
\qquad
n_-\approx \frac{n}{2},
\]
and the sample parent mean satisfies
\[
\bar u\approx 0.
\]
Using the exact reduction formula,
\[
R_{\rm geo}
=
n_+\|\mu_+-\bar u\|^2
+
n_-\|\mu_- -\bar u\|^2 .
\]
Substituting the population approximations gives
\[
R_{\rm geo}
\approx
\frac{n}{2}\frac{2}{\pi}
+
\frac{n}{2}\frac{2}{\pi}.
\]
Hence,
\[
\boxed{
R_{\rm geo}
\approx
\frac{2n}{\pi}.
}
\]

Since
\[
r_0\approx nd,
\]
the geometric split has fractional reduction
\[
\boxed{
\frac{R_{\rm geo}}{r_0}
\approx
\frac{2n/\pi}{nd}
=
\frac{2}{\pi d}.
}
\]

For \(d=3\),
\[
\boxed{
\frac{R_{\rm geo}}{r_0}
\approx
\frac{2}{3\pi}
\approx
0.2122 .
}
\]
Equivalently,
\[
\boxed{
\frac{r_{\rm split,geo}}{r_0}
\approx
1-\frac{2}{3\pi}
\approx
0.7878 .
}
\]


% For the geometric split, define
% \[
% s=v^\top U,
% \qquad
% U\sim \mathcal N(0,I_d).
% \]
% Since \(v\) is a unit vector,
% \[
% s\sim \mathcal N(0,1).
% \]
% The Gaussian distribution is symmetric about zero, so
% \[
% \mathbb P(s>0)=\mathbb P(s<0)=\frac12.
% \]
% Therefore, for \(n\) independent samples,
% \[
% n_+\sim \operatorname{Binomial}\left(n,\frac12\right),
% \qquad
% n_-=n-n_+.
% \]
% Hence,
% \[
% \E[n_+]=\E[n_-]=\frac n2,
% \]
% and by the law of large numbers,
% \[
% \frac{n_+}{n}\to \frac12,
% \qquad
% \frac{n_-}{n}\to \frac12
% \quad
% \text{as } n\to\infty.
% \]
% Thus, for large \(n\),
% \[
% n_+\approx \frac n2,
% \qquad
% n_-\approx \frac n2.
% \]

% Next, the empirical means of the two half-space groups converge to the
% corresponding conditional means:
% \[
% \mu_+
% \to
% \E[U\mid v^\top U>0],
% \qquad
% \mu_-
% \to
% \E[U\mid v^\top U<0].
% \]
% Using the decomposition \(U=sv+z\), where \(z\perp v\), we have
% \[
% \E[U\mid s>0]
% =
% \E[s\mid s>0]v+\E[z\mid s>0].
% \]
% Since the orthogonal component has zero conditional mean,
% \[
% \E[z\mid s>0]=0.
% \]
% Also,
% \[
% \E[s\mid s>0]=\sqrt{\frac{2}{\pi}}.
% \]
% Therefore,
% \[
% \mu_+
% \approx
% \sqrt{\frac{2}{\pi}}v.
% \]
% Similarly,
% \[
% \mu_-
% \approx
% -\sqrt{\frac{2}{\pi}}v.
% \]

% The original unsplit sample mean satisfies
% \[
% \bar u\to \E[U]=0
% \quad
% \text{as } n\to\infty.
% \]
% Therefore, for large \(n\),
% \[
% \bar u\approx 0.
% \]
% Consequently,
% \[
% \|\mu_+-\bar u\|^2
% \approx
% \frac{2}{\pi},
% \qquad
% \|\mu_- -\bar u\|^2
% \approx
% \frac{2}{\pi}.
% \]

% Using the exact reduction formula,
% \[
% R_{\rm geo}
% =
% n_+\|\mu_+-\bar u\|^2
% +
% n_-\|\mu_- -\bar u\|^2,
% \]
% we obtain
% \[
% R_{\rm geo}
% \approx
% \frac n2\frac{2}{\pi}
% +
% \frac n2\frac{2}{\pi}
% =
% \frac{2n}{\pi}.
% \]



